The UN Security Council debates 1992-2023

This paper presents an updated dataset containing 106,302 speeches held in the public meetings of the UN Security Council (UNSC) between 1992 and 2023. The dataset is based on publicly available meeting transcripts with the S/PV document symbol and includes the full substance of individual speeches as well as automatically extracted and manually corrected metadata on the speaker, the position of the speech in the sequence of speeches of a meeting, and the date of the speech. After contextualizing the dataset in recent research on the UNSC, the paper presents descriptive statistics on UNSC meetings and speeches that characterize the period covered by the dataset. Data highlight the extensive presence of the UN bureaucracy in UNSC meetings as well as an emerging trend towards more lengthy open UNSC debates. These open debates cover key issues that have emerged only during the period that is covered by the dataset, for example the debates relating to Women, Peace and Security or Climate-related Disasters. The corpus is available online: https://doi.org/10.7910/DVN/KGVSYH

==> top_25_countries_speeches_total.tex <==
% latex table generated in R 4.4.1 by xtable 1.8-4 package
% Mon Nov  4 09:52:35 2024
\begin{table}[ht]
\centering
\begin{tabular}{lr}
  \hline
country & count \\ 
  \hline
United Kingdom Of Great Britain And Northern Ireland & 5518 \\ 
  United States Of America & 5484 \\ 
  Russian Federation & 5101 \\ 
  France & 4973 \\ 
  China & 4737 \\ 
  UN & 4709 \\ 
  Japan & 2055 \\ 
  Brazil & 1937 \\ 
  Germany & 1928 \\ 
  Mexico & 1412 \\ 
  India & 1371 \\ 
  Spain & 1352 \\ 
  South Africa & 1347 \\ 
  Argentina & 1329 \\ 
  Indonesia & 1208 \\ 
  Pakistan & 1205 \\ 
  Norway & 1121 \\ 
  Nigeria & 1114 \\ 
  Peru & 1102 \\ 
  Poland & 1001 \\ 
  Belgium & 995 \\ 
  Ukraine & 983 \\ 
  Viet Nam & 976 \\ 
  Egypt & 974 \\ 
  Albania & 962 \\ 
   \hline
\end{tabular}
\end{table}

